Learning to Detect Mobile Objects from LiDAR Scans Without Labels

Current 3D object detectors for autonomous driving are almost entirely trained on human-annotated data. Although of high quality, the generation of such data is laborious and costly, restricting them to a few specific locations and object types. This paper proposes an alternative approach entirely based on unlabeled data, which can be collected cheaply and in abundance almost everywhere on earth. Our approach leverages several simple common sense heuristics to create an initial set of approximate seed labels. For example, relevant traffic participants are generally not persistent across multiple traversals of the same route, do not fly, and are never under ground. We demonstrate that these seed labels are highly effective to bootstrap a surprisingly accurate detector through repeated self-training without a single human annotated label.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> supp_figures/self_training_progression.tex <==
{\renewcommand{\tabcolsep}{2pt}
\begin{figure*}[ht]
   \centering
\begin{tabular}{ccc|c}
% \ourmethod (R0) & \ourmethod (R5) & \ourmethod (R10) & \ourmethod (R19) & Ground Truth  \\
\ourmethod (R0) & \ourmethod (R5) & \ourmethod (R10) & Ground Truth  \\
% \hline\hline

\includegraphics[width=0.24\textwidth]{supp_figures/000699_p0_lidar.png}&
\includegraphics[width=0.24\textwidth]{supp_figures/000699_p1_lidar.png}&
\includegraphics[width=0.24\textwidth]{supp_figures/000699_p2_lidar.png}&
% \includegraphics[width=0.19\textwidth]{supp_figures/000699_p9_lidar.png}&
\includegraphics[width=0.24\textwidth]{supp_figures/000699_gt_lidar.png} \\

\includegraphics[width=0.24\textwidth]{supp_figures/012914_p0_lidar.png}&
\includegraphics[width=0.24\textwidth]{supp_figures/012914_p1_lidar.png}&
\includegraphics[width=0.24\textwidth]{supp_figures/012914_p2_lidar.png}&
% \includegraphics[width=0.19\textwidth]{supp_figures/012914_p9_lidar.png}&
\includegraphics[width=0.24\textwidth]{supp_figures/012914_gt_lidar.png} 
% \includegraphics[width=0.15\textwidth,height=0.15\textwidth]{figures/day2night_qualitative/img95_input.png}&
% \includegraphics[width=0.15\textwidth,height=0.15\textwidth]{figures/day2night_qualitative/img95_gt.png}&
% \includegraphics[width=0.15\textwidth,height=0.15\textwidth]{figures/day2night_qualitative/img95_scratch.png}&
% \includegraphics[width=0.15\textwidth,height=0.15\textwidth]{figures/day2night_qualitative/img95_finetune.png}&
% \includegraphics[width=0.15\textwidth,height=0.15\textwidth]{figures/day2night_qualitative/img95_baseline.png}&
% \includegraphics[width=0.15\textwidth,height=0.15\textwidth]{figures/day2night_qualitative/img95_method.png}


\end{tabular}

\caption{Visual comparison of self-training iteration results on \ourmethod.
% For Satellite$\rightarrow$Map (top 3) our method out-performs the baselines visually and is very close to the ground truth. Map$\rightarrow$Satellite (bottom 3) our method reduces the ghosting artifacts present in the other methods.
}
\label{fig:st_progression}
\vspace{-15pt}
\end{figure*}
}

==> supp_tables/main_dynamic.tex <==
\begin{table*}[!th]
\centering
\renewcommand{\arraystretch}{1.05}
\tabcolsep 2pt
\caption{\textbf{Detection performance with different methods on the \lyft dataset.} 
Please refer to \autoref{tbl:main} for naming.
\label{tbl:main_supp}}
% \vspace{-5pt}
\begin{tabular}{=l|+C{44pt}|+C{44pt}|+C{44pt}||+C{44pt}||+C{44pt}|+C{44pt}|+C{44pt}||+C{44pt}}
\multicolumn{1}{c|}{\multirow{2}{*}{Method}} & \multicolumn{4}{c||}{\APBEV / \AP @ IoU = 0.25} &  \multicolumn{4}{c}{\APBEV / \AP @ IoU = 0.5}\\
\cline{2-9}\
 & 0-30 & 30-50 & 50-80 & 0-80 & 0-30 & 30-50 & 50-80 & 0-80\\\hline
%  \ourmethod-\pp (R0)
%  & 46.4 / 45.4 & 16.5 / 10.8 & \phantom{0}0.9 / \phantom{0}0.4 & 21.8 / 18.0 
%  & 34.1 / 31.3 & \phantom{0}5.1 / \phantom{0}3.0 & \phantom{0}0.0 / \phantom{0}0.0 & 12.0 / \phantom{0}9.7 \\
%  \ourmethod-\pp (R10)
%  & 49.9 / 49.3 & 32.3 / 27.0 & \phantom{0}3.5 /\phantom{0} 1.4 & 30.9 / 27.3 
%  & 42.1 / 38.3 & 21.9 / 19.2 & \phantom{0}1.0 / \phantom{0}0.9 & 22.8 / 20.6
%  \\
 \ourmethod (R0)
 & 65.7 / 63.0 & 41.4 / 36.0 & \phantom{0}8.9 / \phantom{0}5.7 & 42.5 / 37.9 
 & 44.9 / 40.4 & 24.5 / 14.8 & \phantom{0}2.7 / \phantom{0}0.7 & 26.3 / 19.8 \\
 \ourmethod (R10)
 & 73.8 / 71.3 & 62.8 / 60.3 & 27.0 / 24.8 & 57.3 / 55.1 
 & 56.8 / 51.3 & 51.4 / 40.5 & 19.2 / \phantom{0}9.0 & 44.1 / 35.5 \\
 \ourmethod (R17)\textsuperscript{\ref{footnote:20ptc}}
%  \tablefootnote{By the time of submission this is the model trained with most rounds of self-training (by using 20\% of unlabeled data). We will update \ourmethod (R20 & 100\%) in the camera ready version.}
 & 75.7 / 73.6 & 62.7 / 61.9 & 34.0 / 32.6 & 59.6 / 57.8
 & 58.4 / 53.0 & 55.0 / 46.6 & 28.8 / 17.8 & 48.4 / 40.5 \\
 \ourmethod (R30)
%  \tablefootnote{By the time of submission this is the model trained with most rounds of self-training (by using 20\% of unlabeled data). We will update \ourmethod (R20 & 100\%) in the camera ready version.}
 & 76.2 / 74.1 & 64.3 / 62.9 & 45.4 / 43.9 & 63.3 / 61.6
 & 61.2 / 55.7 & 57.4 / 52.3 & 40.2 / 28.2 & 53.8 / 46.4\\
\hline\hline
\rowstyle{\leavevmode\color{gray}} Sup. (\kitti) 
& 79.3 / 78.9 & 57.2 / 56.6 & 30.8 / 29.8 & 58.6 / 57.3 
& 72.3 / 69.5 & 53.2 / 48.1 & 27.9 / 20.5 & 53.1 / 48.1  \\
\rowstyle{\leavevmode\color{gray}} Sup. (\lyft)
& 82.8 / 82.6 & 70.8 / 70.3 & 50.2 / 49.6 & 69.5 / 69.1 
& 79.6 / 77.5 & 66.4 / 64.4& 47.8 / 43.8 & 65.5 / 63.2  \\
 \hline
\end{tabular}
\vspace{-10pt}
\end{table*}


==> tables/main_dynamic.tex <==
\begin{table*}[!th]
\centering
\renewcommand{\arraystretch}{1.05}
\tabcolsep 2pt
\caption{\textbf{Detection performance with different methods on the \lyft dataset.} 
% \YY{TODO: update the results on Monday!}
We report \APBEV / \AP with IoU=$0.5$ and IoU=$0.25$ for mobile objects under various ranges.
% CS stands for with common-sense rules except \pp, 
R$i$ stands for $i$-th round self-training (R0 is training from seed labels). 
We also report the performance of detectors trained with ground-truth labels on the \kitti and the \lyft datasets at the last two rows. 
% \todo{Update with R40 results}
\vspace{-5pt}
\label{tbl:main}}
\begin{tabular}{=l|+C{44pt}|+C{44pt}|+C{44pt}||+C{44pt}||+C{44pt}|+C{44pt}|+C{44pt}||+C{44pt}}
\multicolumn{1}{c|}{\multirow{2}{*}{Method}} & \multicolumn{4}{c||}{\APBEV / \AP @ IoU = 0.25} &  \multicolumn{4}{c}{\APBEV / \AP @ IoU = 0.5}\\
\cline{2-9}\
 & 0-30 & 30-50 & 50-80 & 0-80 & 0-30 & 30-50 & 50-80 & 0-80\\\hline
 \ourmethod-\pp (R0)
 & 46.4 / 45.4 & 16.5 / 10.8 & \phantom{0}0.9 / \phantom{0}0.4 & 21.8 / 18.0 
 & 34.1 / 31.3 & \phantom{0}5.1 / \phantom{0}3.0 & \phantom{0}0.0 / \phantom{0}0.0 & 12.0 / \phantom{0}9.7 \\
 \ourmethod-\pp (R10)
 & 49.9 / 49.3 & 32.3 / 27.0 & \phantom{0}3.5 /\phantom{0} 1.4 & 30.9 / 27.3 
 & 42.1 / 38.3 & 21.9 / 19.2 & \phantom{0}1.0 / \phantom{0}0.9 & 22.8 / 20.6
 \\
 \ourmethod (R0)
 & 65.7 / 63.0 & 41.4 / 36.0 & \phantom{0}8.9 / \phantom{0}5.7 & 42.5 / 37.9 
 & 44.9 / 40.4 & 24.5 / 14.8 & \phantom{0}2.7 / \phantom{0}0.7 & 26.3 / 19.8 \\
 \ourmethod (R10)
 & 73.8 / 71.3 & 62.8 / 60.3 & 27.0 / 24.8 & 57.3 / 55.1 
 & 56.8 / 51.3 & 51.4 / 40.5 & 19.2 / \phantom{0}9.0 & 44.1 / 35.5 \\
 \ourmethod (R40)
%  \tablefootnote{By the time of submission this is the model trained with most rounds of self-training (by using 20\% of unlabeled data). We will update \ourmethod (R20, 100\%) in the camera ready version.}
 & 76.4 / 74.1 & 64.2 / 62.9 & 47.1 / 45.5 & 64.4 / 62.7
 & 61.1 / 56.2 & 57.5 / 53.4 & 41.2 / 29.8 & 54.1 / 47.6 \\
\hline\hline
\rowstyle{\leavevmode\color{gray}} Sup. (\kitti) 
& 79.3 / 78.9 & 57.2 / 56.6 & 30.8 / 29.8 & 58.6 / 57.3 
& 72.3 / 69.5 & 53.2 / 48.1 & 27.9 / 20.5 & 53.1 / 48.1  \\
\rowstyle{\leavevmode\color{gray}} Sup. (\lyft)
& 82.8 / 82.6 & 70.8 / 70.3 & 50.2 / 49.6 & 69.5 / 69.1 
& 79.6 / 77.5 & 66.4 / 64.4& 47.8 / 43.8 & 65.5 / 63.2  \\
 \hline
\end{tabular}
\vspace{-10pt}
\end{table*}

